Imitating Human Behaviour with Diffusion Models

Diffusion models have emerged as powerful generative models in the text-to-image domain. This paper studies their application as observation-to-action models for imitating human behaviour in sequential environments. Human behaviour is stochastic and multimodal, with structured correlations between action dimensions. Meanwhile, standard modelling choices in behaviour cloning are limited in their expressiveness and may introduce bias into the cloned policy. We begin by pointing out the limitations of these choices. We then propose that diffusion models are an excellent fit for imitating human behaviour, since they learn an expressive distribution over the joint action space. We introduce several innovations to make diffusion models suitable for sequential environments; designing suitable architectures, investigating the role of guidance, and developing reliable sampling strategies. Experimentally, diffusion models closely match human demonstrations in a simulated robotic control task and a modern 3D gaming environment.

==> 02_table_figs_etc/tbl_kitchen_mainpaper.tex <==
\begin{table}[h!]
\begin{center}
\label{tbl_kitchen_results}
\caption{Robotic control results. Mean $\pm$ one standard error over three training runs (100$\times$rollouts).}
\vspace{0.2in}
\resizebox{0.9 \columnwidth}{!}{
\begin{tabular}{lrrrrrrr}
{} &   Tasks $\geq$ 1 &  Tasks $\geq$ 2 &  Tasks $\geq$ 3 &  Tasks $\geq$ 4  &  Tasks Wasserstein & Time-taken Wasserstein\\ \hline\\
\midrule

Diffusion BC, Basic MLP         &  0.98 pm 0.01 &  0.89 pm 0.01 &   0.71 pm 0.0 &  0.45 pm 0.03 &      1.96 pm 0.12 & 12.04 $\pm$ 2.20\\
Diffusion-KDE, Basic MLP    &   0.99 pm 0.0 &  0.97 pm 0.01 &   0.86 pm 0.0 &  0.59 pm 0.01 &      1.72 pm 0.03 & 8.08 $\pm$ 0.24\\
Diffusion-X, Basic MLP  &  0.99 pm 0.01 &  0.93 pm 0.01 &  0.83 pm 0.02 &  0.58 pm 0.02 &      1.51 pm 0.14 & 8.61 $\pm$ 0.14\\

\\
% \\ MLP architecture \\
MSE, MLP Sieve                     &   0.99 $\pm$ 0.0 &   0.9 $\pm$ 0.03 &  0.72 $\pm$ 0.03 &   0.5 $\pm$ 0.02 &   1.91 $\pm$ 0.07 & 6.40 $\pm$ 0.48\\
Discretised, MLP Sieve             &  0.95 $\pm$ 0.02 &  0.73 $\pm$ 0.02 &   0.4 $\pm$ 0.03 &  0.18 $\pm$ 0.02 &    3.43 $\pm$ 0.14 & 11.30 $\pm$ 1.29\\
K-Means, MLP Sieve           &   0.3 $\pm$ 0.03 &   0.03 $\pm$ 0.0 &    0.0 $\pm$ 0.0 &    0.0 $\pm$ 0.0 &    5.25 $\pm$ 0.0 & --\\
K-Means+Residual, MLP Sieve   &  0.95 $\pm$ 0.0 &  0.82 $\pm$ 0.01 &  0.55 $\pm$ 0.02 &  0.23 $\pm$ 0.02 &  2.87 $\pm$ 0.16 & 11.60 $\pm$ 2.11\\
Diffusion BC, MLP Sieve         &  0.99 $\pm$ 0.0 &  0.94 $\pm$ 0.0 &  0.82 $\pm$ 0.02 &  0.68 $\pm$ 0.02 &  1.31 $\pm$ 0.05 & 6.06 $\pm$ 1.10\\
Diffusion-KDE, MLP Sieve     &   1.0 $\pm$ 0.0 &   1.0 $\pm$ 0.0 &  0.92 $\pm$ 0.01 &  0.79 $\pm$ 0.04 &  1.6 $\pm$ 0.24 & 6.77 $\pm$ 0.64\\
Diffusion-X, MLP Sieve  &   1.0 $\pm$ 0.0 &  0.97 $\pm$ 0.0 &   0.9 $\pm$ 0.01 &  0.77 $\pm$ 0.02 &   1.06 $\pm$ 0.05 & 5.24 $\pm$ 0.90\\


\\
% \\ Transformer architecture \\
MSE, Transformer              &   0.99 $\pm$ 0.0 &  0.96 $\pm$ 0.01 &  0.88 $\pm$ 0.01 &  0.69 $\pm$ 0.02 &  1.47 $\pm$ 0.13  & 5.85 $\pm$ 0.27\\
Discretised, Transformer      &   0.97 $\pm$ 0.0 &  0.82 $\pm$ 0.02 &  0.57 $\pm$ 0.04 &  0.34 $\pm$ 0.02 &  2.54 $\pm$ 0.14 & 6.13 $\pm$ 0.49\\
K-Means, Transformer    &   0.42 &   0.05 &    0.0 &    0.0 &    5.25  & --\\
K-Means+Residual, Transformer  &   0.98 $\pm$ 0.0 &  0.91 $\pm$ 0.01 &  0.66 $\pm$ 0.04 &  0.34 $\pm$ 0.02 &  2.25 $\pm$ 0.16 & 7.80 $\pm$ 0.87\\  
Diffusion BC, Transformer        &    1.0 $\pm$ 0.0 &  0.98 $\pm$ 0.01 &   0.9 $\pm$ 0.02 &  0.77 $\pm$ 0.01 &   1.35 $\pm$ 0.11 & 4.11 $\pm$ 0.05\\
Diffusion-KDE, Transformer   &    1.0 $\pm$ 0.0 &    1.0 $\pm$ 0.0 &   0.95 $\pm$ 0.0 &  0.89 $\pm$ 0.01 &   1.31 $\pm$ 0.03 & 5.28 $\pm$ 0.41\\
Diffusion-X, Transformer  &    1.0 $\pm$ 0.0 &  0.99 $\pm$ 0.01 &   0.94 $\pm$ 0.0 &  0.88 $\pm$ 0.01 &   1.17 $\pm$ 0.13 & 4.65 $\pm$ 0.47\\

\\ Previously reported \\
Behaviour Transformers & 0.99 & 0.93 & 0.71 & 0.44 & -- & --\\
Implicit BC & 0.99 & 0.87 & 0.61 & 0.24 & -- & --\\


\\ Baselines \\
Human                          &    1.0 $\pm$ 0.0 &   1.0 $\pm$ 0.0 &    1.0 $\pm$ 0.0 &   0.98 $\pm$ 0.0 &    0.0 $\pm$ 0.0 & --\\
Human subsampled               &    1.0 $\pm$ 0.0 &   1.0 $\pm$ 0.0 &    1.0 $\pm$ 0.0 &   0.98 $\pm$ 0.0 &    0.82 $\pm$ 0.04 & --\\


\bottomrule
\end{tabular}
}
\end{center}
\end{table}

These are the results (so far) for the Wasserstein between the trajectories and dataset.
\begin{table}[h!]
\begin{center}
\label{tbl_kitchen_results_wass}
\caption{Robotic control results. Mean $\pm$ one standard error over three training runs (100$\times$rollouts).}
\vspace{0.2in}

\begin{tabular}{lr}
{} &  Wasserstein \\ \hline\\
\midrule

Diffusion-Extra MLP Basic & 0.424 $\pm$ 0.017 \\
Diffusion MLP Basic & 0.463 $\pm$ 0.012 \\
Diffusion-KDE Basic MLP & 0.481 $\pm$ 0.005 \\
\\
MSE MLP &   0.443 $\pm$ 0.021 \\
Discretised MLP &   0.651 $\pm$ 0.026 \\
K-Means MLP &   1.469 $\pm$ 0.120 \\
K-Means+Residual MLP &   0.607 $\pm$ 0.027 \\
Diffusion MLP &   0.373 $\pm$ 0.012 \\
Diffusion-KDE MLP &   0.439 $\pm$ 0.039 \\
Diffusion-Extra MLP &   0.344 $\pm$ 0.004 \\
\\
MSE Transformer &   0.397 $\pm$ 0.034 \\
Discretised Transformer &   0.512 $\pm$ 0.002 \\
K-Means Transformer &   1.470 \footnote{1 run only}\\
K-Means+Residual Transformer &   0.426 $\pm$ 0.018 \\
Diffusion Transformer &   0.340 $\pm$ 0.003 \\
Diffusion-KDE Transformer &   0.418 $\pm$ 0.012 \\
Diffusion-Extra Transformer &   0.365 $\pm$ 0.013 \\
\\
Human sub-sampled & 0.223 $\pm$ 0.006 \\

\bottomrule
\end{tabular}

\end{center}
\end{table}

==> 02_table_figs_etc/tbl_kitchen_prdc.tex <==
\begin{table}[h!]
\begin{center}
\label{tbl_kitchen_prdc}
\caption{Density and Coverage metrics with 10 nearest neighbours}
\begin{tabular}{lrr}
{} &  Density & Coverage \\ \hline\\

Diffusion-Extra MLP Basic &  0.64 $\pm$ 0.00 & 0.41 $\pm$ 0.00 \\
Diffusion MLP Basic &  0.54 $\pm$ 0.02 & 0.38 $\pm$ 0.01 \\
Diffusion-KDE MLP Basic &  0.78 $\pm$ 0.00 & 0.37 $\pm$ 0.00 \\
\\
% \midrule
MSE MLP &  0.71 $\pm$ 0.01 & 0.40 $\pm$ 0.01 \\
Discrete MLP &  0.38 $\pm$ 0.02 & 0.31 $\pm$ 0.01 \\
K-Means MLP &  0.09 $\pm$ 0.00 & 0.06 $\pm$ 0.00 \\
K-Means+Residual MLP &  0.51 $\pm$ 0.01 & 0.36 $\pm$ 0.00 \\
Diffusion MLP &  0.66 $\pm$ 0.01 & 0.42 $\pm$ 0.00 \\
Diffusion-KDE MLP &  0.93 $\pm$ 0.02 & 0.41 $\pm$ 0.01 \\
Diffusion-Extra MLP &  0.78 $\pm$ 0.01 & 0.45 $\pm$ 0.00 \\

\\

MSE Transformer &  0.81 $\pm$ 0.01 & 0.42 $\pm$ 0.01 \\
Discrete Transformer &  0.47 $\pm$ 0.01 & 0.36 $\pm$ 0.00 \\ 
K-Means Transformer &  0.07 & 0.06 \\
K-Means+Residual Transformer &  0.66 $\pm$ 0.02 & 0.38 $\pm$ 0.01 \\
Diffusion-Extra Transformer &  0.94 $\pm$ 0.02 & 0.45 $\pm$ 0.01 \\
Diffusion Transformer &  0.74 $\pm$ 0.01 & 0.44 $\pm$ 0.00 \\
Diffusion-KDE Transformer &  0.97 $\pm$ 0.02 & 0.43 $\pm$ 0.01 \\
\\
Human &  1.00 $\pm$ 0.01 & 0.56 $\pm$ 0.01 \\

% \bottomrule
\end{tabular}

\end{center}
\end{table}

